Dynamic detection of mobile malware using smartphone data and machine learning

Mobile malware are malicious programs that target mobile devices. They are an increasing problem, as seen in the rise of detected mobile malware samples per year. The number of active smartphone users is expected to grow, stressing the importance of research on the detection of mobile malware. Detection methods for mobile malware exist but are still limited. In this paper, we provide an overview of the performance of machine learning (ML) techniques to detect malware on Android, without using privileged access. The ML-classifiers use device information such as the CPU usage, battery usage, and memory usage for the detection of 10 subtypes of Mobile Trojans on the Android Operating System (OS). We use a real-life dataset containing device and malware data from 47 users for a year (2016). We examine which features, i.e. aspects, of a device, are most important to monitor to detect (subtypes of) Mobile Trojans. The focus of this paper is on dynamic hardware features. Using these dynamic features we apply state-of-the-art machine learning classifiers: Random Forest, K-Nearest Neighbour, and AdaBoost. We show classification results on different feature sets, making a distinction between global device features, and specific app features. None of the measured feature sets require privileged access. Our results show that the Random Forest classifier performs best as a general malware classifier: across 10 subtypes of Mobile Trojans, it achieves an F1 score of 0.73 with a False Positive Rate (FPR) of 0.009 and a False Negative Rate (FNR) of 0.380. The Random Forest, K-Nearest Neighbours, and AdaBoost classifiers achieve F1 scores above 0.72, an FPR below 0.02 and, an FNR below 0.33, when trained separately to detect each subtype of Mobile Trojans.

==> comparison_classifier_allclassifiers.tex <==
% Preview source code for paragraph 0
\begin{tabular}{lccccccccccccccc}
\toprule
\textbf{Classifier} & \multicolumn{3}{c}{\textbf{AdaBoost}} & \multicolumn{3}{c}{\textbf{Random Forest}} & \multicolumn{3}{c}{\textbf{KNN}} & \multicolumn{3}{c}{\textbf{Na\"{i}ve Bayes}} & \multicolumn{3}{c}{\textbf{MLP}}\tabularnewline
Featureset & fs1 & fs2 & fs3 & fs1 & fs2 & fs3 & fs1 & fs2 & fs3 & fs1 & fs2 & fs3 & fs1 & fs2 & fs3\tabularnewline

%\cmidrule(lr){2-4}\cmidrule(lr){5-7}\cmidrule(lr){8-10}\cmidrule(lr){11-13}\cmidrule(lr){14-16}
\tabularnewline
\multicolumn{16}{l}{\textbf{Best model}}\tabularnewline
\cmidrule(lr){2-4}\cmidrule(lr){5-7}\cmidrule(lr){8-10}\cmidrule(lr){11-13}\cmidrule(lr){14-16}
Nr. features & 26 & 25 & 43 & 24 & 29 & 10 & 26 & 13 & 9 & 31 & 33 & 64 & 32 & 28 & 62\tabularnewline
Accuracy & 0.922 & 0.943 & 0.945 & 0.922 & 0.958 & 0.959 & 0.897 & 0.944 & 0.946 & 0.913 & 0.920 & 0.919 & 0.913 & 0.937 & 0.940\tabularnewline
f1 score & 0.226 & 0.595 & 0.610 & 0.422 & 0.730 & 0.722 & 0.356 & 0.674 & 0.688 & 0.000 & 0.343 & 0.351 & 0.000 & 0.493 & 0.567\tabularnewline
fpr & 0.003 & 0.012 & 0.013 & 0.022 & 0.013 & 0.009 & 0.048 & 0.029 & 0.028 & 0.000 & 0.015 & 0.017 & 0.000 & 0.007 & 0.014\tabularnewline
fnr & 0.868 & 0.522 & 0.502 & 0.670 & 0.346 & 0.380 & 0.674 & 0.336 & 0.320 & 1.000 & 0.760 & 0.748 & 1.000 & 0.648 & 0.546\tabularnewline
 &  &  &  &  &  &  &  &  &  &  &  &  &  &  & \tabularnewline
\multicolumn{16}{l}{\textbf{Feature categories used}}\tabularnewline
\cmidrule(lr){2-4}\cmidrule(lr){5-7}\cmidrule(lr){8-10}\cmidrule(lr){11-13}\cmidrule(lr){14-16}
Battery & X &  & X & X &  &  & X &  &  & X &  & X & X &  & X\tabularnewline
CPU & X &  & X & X &  &  & X &  &  & X &  & X & X &  & X\tabularnewline
I/O Interrupts &  &  &  &  &  &  &  &  &  &  &  &  &  &  & \tabularnewline
Memory & X &  & X & X &  &  & X &  &  & X &  & X & X &  & X\tabularnewline
Network traff. & X &  & X & X &  &  & X &  &  & X &  & X & X &  & X\tabularnewline
Storage &  &  &  &  &  &  &  &  &  &  &  &  &  &  & \tabularnewline
Wifi &  &  &  &  &  &  &  &  &  &  &  &  &  &  & \tabularnewline
App CPU &  & X & X &  & X & X &  & X & X &  & X & X &  & X & X\tabularnewline
App memory &  & X & X &  & X & X &  & X & X &  & X & X &  & X & X\tabularnewline
App netw. traff. &  & X & X &  & X &  &  & X &  &  & X & X &  & X & X\tabularnewline
App process &  & X & X &  & X & X &  & X & X &  & X & X &  & X & X\tabularnewline
\bottomrule
\end{tabular}


==> comparison_classifiers2.tex <==
% Preview source code for paragraph 0
\begin{tabularx}{\textwidth}{lCCCCCCCCC}
\toprule
\textbf{Classifier} & \multicolumn{3}{c}{\textbf{AdaBoost}} & \multicolumn{3}{c}{\textbf{Random Forest}} & \multicolumn{3}{c}{\textbf{KNN}} \tabularnewline
\textbf{Feature set} & Global & Apps & Comb. & Global & \textbf{Apps} & Comb. & Global & Apps & Comb. \tabularnewline

%\cmidrule(lr){2-4}\cmidrule(lr){5-7}\cmidrule(lr){8-10}\cmidrule(lr){11-13}\cmidrule(lr){14-16}
%\tabularnewline
\multicolumn{10}{l}{\textbf{Best trained model}}\tabularnewline
\cmidrule(lr){2-4}\cmidrule(lr){5-7}\cmidrule(lr){8-10}
Nr. features & 26 & 25 & 43 & 24 & \textbf{29} & 10 & 26 & 13 & 9\tabularnewline
Accuracy & 0.922 & 0.943 & 0.945 & 0.922 & \textbf{0.958} & 0.959 & 0.897 & 0.944 & 0.946\tabularnewline
F1 score & 0.226 & 0.595 & 0.610 & 0.422 & \textbf{0.730} & 0.722 & 0.356 & 0.674 & 0.688\tabularnewline
FPR & 0.003 & 0.012 & 0.013 & 0.022 & \textbf{0.013} & 0.009 & 0.048 & 0.029 & 0.028\tabularnewline
FNR & 0.868 & 0.522 & 0.502 & 0.670 & \textbf{0.346} & 0.380 & 0.674 & 0.336 & 0.320\tabularnewline
\multicolumn{10}{l}{\textbf{Feature categories used}}\tabularnewline
\cmidrule(lr){2-4}\cmidrule(lr){5-7}\cmidrule(lr){8-10}
Battery & v &  & v & v &  &  & v &  & \tabularnewline
CPU & v &  & v & v &  &  & v &  & \tabularnewline
IO Interrupts &  &  &  &  &  &  &  &  & \tabularnewline
Memory & v &  & v & v &  &  & v &  & \tabularnewline
Metadata &  &  &  &  &  &  &  &  & \tabularnewline
Network & v &  & v & v &  &  & v &  & \tabularnewline
Storage &  &  &  &  &  &  &  &  & \tabularnewline
Wifi &  &  &  &  &  &  &  &  & \tabularnewline
App CPU &  & v & v &  & \textbf{v} & v &  & v & v\tabularnewline
App Info &  &  &  &  &  &  &  &  & \tabularnewline
App Memory &  & v & v &  & \textbf{v} & v &  & v & v\tabularnewline
App Network traffic &  & v & v &  & \textbf{v} &  &  & v & \tabularnewline
App Process &  & v & v &  & \textbf{v} & v &  & v & v\tabularnewline
\bottomrule
\end{tabularx}


==> experiments_overview.tex <==
% Preview source code for paragraph 0

\begin{tabularx}{\textwidth}{lLll}
\hline
\textbf{Classifier} & \textbf{Featureset} & \textbf{Training mode} & \textbf{Testing mode} \tabularnewline
\hline
\textbf{Random Forest} & Global & All & Normal holdout\tabularnewline
 %\cmidrule(l){0-0}\cmidrule(l){2-2}\cmidrule(l){3-3}
\hline
\textbf{K-Nearest Neighbour} & Apps & Per mwtype & Unknown device \tabularnewline
%\cmidrule(l){0-0}\cmidrule(l){2-2}\cmidrule(l){3-3}
\hline
\textbf{AdaBoost} & Combined  \tabularnewline
\hline
\end{tabularx}


==> experiments_overview2.tex <==
% Preview source code for paragraph 0

\begin{tabularx}{\textwidth}{lLLL}
\toprule
\textbf{Classifier} & \textbf{Featuresets} & \textbf{Training modes} & \textbf{Test modes} \tabularnewline
\hline
\textbf{Random Forest} & Global, Apps, Combined & All, Per mwtype & Normal holdout, Unknown device \tabularnewline
 %\cmidrule(l){0-0}\cmidrule(l){2-2}\cmidrule(l){3-3}
\hline
\textbf{K-Nearest Neighbour} &  Global, Apps, Combined & All, Per mwtype  & Normal holdout, Unknown device \tabularnewline
%\cmidrule(l){0-0}\cmidrule(l){2-2}\cmidrule(l){3-3}
\hline
\textbf{AdaBoost} &  Global, Apps, Combined & All, Per mwtype  & Normal holdout, Unknown device   \tabularnewline
\bottomrule
\end{tabularx}


==> search_space.tex <==
% Preview source code for paragraph 0

\begin{tabularx}{\textwidth}{lll}
\toprule
\textbf{Classifier} & \textbf{Parameter} & \textbf{Search space}  \tabularnewline
\hline
\textbf{Random Forest} & Number of estimators & [5, 10, 20, 50, 100, 200, 400] \tabularnewline
 & Maximum depth tree & [3, 5, 10, 20, 40, 80, 160, 320] \tabularnewline
 & Maximum features  & [3, 5 10, 20, 40, 60, 80, 100, 120, 140, 171] \tabularnewline
 %\cmidrule(l){0-0}\cmidrule(l){2-2}\cmidrule(l){3-3}
\hline
\textbf{K-Nearest Neighbour} & Number of neighbours & [1, 3, 7, 11, 21, 31, 61]
 \tabularnewline
%\cmidrule(l){0-0}\cmidrule(l){2-2}\cmidrule(l){3-3}
\hline
\textbf{AdaBoost} & Number of estimators & [3, 5 10, 20, 40, 60, 80, 100, 120, 140, 171]  \tabularnewline
\bottomrule
\end{tabularx}

